LPGNet: Link Private Graph Networks for Node Classification

Classification tasks on labeled graph-structured data have many important applications ranging from social recommendation to financial modeling. Deep neural networks are increasingly being used for node classification on graphs, wherein nodes with similar features have to be given the same label. Graph convolutional networks (GCNs) are one such widely studied neural network architecture that perform well on this task. However, powerful link-stealing attacks on GCNs have recently shown that even with black-box access to the trained model, inferring which links (or edges) are present in the training graph is practical. In this paper, we present a new neural network architecture called LPGNet for training on graphs with privacy-sensitive edges. LPGNet provides differential privacy (DP) guarantees for edges using a novel design for how graph edge structure is used during training. We empirically show that LPGNet models often lie in the sweet spot between providing privacy and utility: They can offer better utility than "trivially" private architectures which use no edge information (e.g., vanilla MLPs) and better resilience against existing link-stealing attacks than vanilla GCNs which use the full edge structure. LPGNet also offers consistently better privacy-utility tradeoffs than DPGCN, which is the state-of-the-art mechanism for retrofitting differential privacy into conventional GCNs, in most of our evaluated datasets.

==> chapters/appendices/Nl-1_2_Cora.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the transductive setting using the micro-average F1 score on Cora Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.6 \pm 0.0$ & $0.52 \pm 0.02$ & $ - $ & $0.81 \pm 0.0$ & $0.34 \pm 0.03$\\
2.0 & $0.6 \pm 0.0$ & $0.59 \pm 0.01$ & $0.56 \pm 0.02$ & $0.81 \pm 0.0$ & $0.35 \pm 0.02$\\
3.0 & $0.6 \pm 0.0$ & $0.63 \pm 0.02$ & $ - $ & $0.81 \pm 0.0$ & $0.35 \pm 0.02$\\
4.0 & $0.6 \pm 0.0$ & $0.65 \pm 0.02$ & $0.64 \pm 0.01$ & $0.81 \pm 0.0$ & $0.37 \pm 0.02$\\
5.0 & $0.6 \pm 0.0$ & $0.67 \pm 0.02$ & $ - $ & $0.81 \pm 0.0$ & $0.42 \pm 0.02$\\
6.0 & $0.6 \pm 0.0$ & $0.68 \pm 0.01$ & $0.68 \pm 0.01$ & $0.81 \pm 0.0$ & $0.53 \pm 0.02$\\
7.0 & $0.6 \pm 0.0$ & $0.68 \pm 0.01$ & $ - $ & $0.81 \pm 0.0$ & $0.66 \pm 0.01$\\
8.0 & $0.6 \pm 0.0$ & $0.69 \pm 0.02$ & $0.7 \pm 0.01$ & $0.81 \pm 0.0$ & $0.72 \pm 0.01$\\
9.0 & $0.6 \pm 0.0$ & $0.69 \pm 0.01$ & $ - $ & $0.81 \pm 0.0$ & $0.76 \pm 0.01$\\
10.0 & $0.6 \pm 0.0$ & $0.69 \pm 0.02$ & $0.71 \pm 0.01$ & $0.81 \pm 0.0$ & $0.78 \pm 0.01$\\
\hline
\end{tabular}
 }
\label{tab:cora-dp-ind}
\end{table}

==> chapters/appendices/Nl-1_2_PubMed.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the transductive setting using the micro-average F1 score on Pubmed Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.72 \pm 0.01$ & $0.71 \pm 0.01$ & $ - $ & $0.79 \pm 0.0$ & $0.55 \pm 0.02$\\
2.0 & $0.72 \pm 0.01$ & $0.73 \pm 0.01$ & $0.71 \pm 0.02$ & $0.79 \pm 0.0$ & $0.55 \pm 0.02$\\
3.0 & $0.72 \pm 0.01$ & $0.73 \pm 0.01$ & $ - $ & $0.79 \pm 0.0$ & $0.55 \pm 0.02$\\
4.0 & $0.72 \pm 0.01$ & $0.74 \pm 0.01$ & $0.73 \pm 0.01$ & $0.79 \pm 0.0$ & $0.55 \pm 0.02$\\
5.0 & $0.72 \pm 0.01$ & $0.74 \pm 0.0$ & $ - $ & $0.79 \pm 0.0$ & $0.55 \pm 0.02$\\
6.0 & $0.72 \pm 0.01$ & $0.74 \pm 0.01$ & $0.74 \pm 0.01$ & $0.79 \pm 0.0$ & $0.56 \pm 0.02$\\
7.0 & $0.72 \pm 0.01$ & $0.74 \pm 0.0$ & $ - $ & $0.79 \pm 0.0$ & $0.59 \pm 0.02$\\
8.0 & $0.72 \pm 0.01$ & $0.74 \pm 0.0$ & $0.74 \pm 0.01$ & $0.79 \pm 0.0$ & $0.64 \pm 0.02$\\
9.0 & $0.72 \pm 0.01$ & $0.74 \pm 0.0$ & $ - $ & $0.79 \pm 0.0$ & $0.69 \pm 0.02$\\
10.0 & $0.72 \pm 0.01$ & $0.74 \pm 0.0$ & $0.75 \pm 0.01$ & $0.79 \pm 0.0$ & $0.73 \pm 0.02$\\
\hline
\end{tabular}
 }
\label{tab:pubmed-dp-ind}
\end{table}

==> chapters/appendices/Nl1_2-Citeseer.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the transductive setting using the micro-average F1 score on Citeseer Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.6 \pm 0.01$ & $0.58 \pm 0.02$ & $ - $ & $0.72 \pm 0.0$ & $0.36 \pm 0.02$\\
2.0 & $0.6 \pm 0.01$ & $0.62 \pm 0.01$ & $0.55 \pm 0.02$ & $0.72 \pm 0.0$ & $0.36 \pm 0.02$\\
3.0 & $0.6 \pm 0.01$ & $0.63 \pm 0.01$ & $ - $ & $0.72 \pm 0.0$ & $0.37 \pm 0.01$\\
4.0 & $0.6 \pm 0.01$ & $0.64 \pm 0.01$ & $0.62 \pm 0.01$ & $0.72 \pm 0.0$ & $0.38 \pm 0.02$\\
5.0 & $0.6 \pm 0.01$ & $0.64 \pm 0.01$ & $ - $ & $0.72 \pm 0.0$ & $0.41 \pm 0.02$\\
6.0 & $0.6 \pm 0.01$ & $0.64 \pm 0.01$ & $0.64 \pm 0.01$ & $0.72 \pm 0.0$ & $0.46 \pm 0.02$\\
7.0 & $0.6 \pm 0.01$ & $0.64 \pm 0.01$ & $ - $ & $0.72 \pm 0.0$ & $0.55 \pm 0.02$\\
8.0 & $0.6 \pm 0.01$ & $0.65 \pm 0.01$ & $0.65 \pm 0.01$ & $0.72 \pm 0.0$ & $0.62 \pm 0.02$\\
9.0 & $0.6 \pm 0.01$ & $0.65 \pm 0.01$ & $ - $ & $0.72 \pm 0.0$ & $0.67 \pm 0.01$\\
10.0 & $0.6 \pm 0.01$ & $0.65 \pm 0.01$ & $0.65 \pm 0.01$ & $0.72 \pm 0.0$ & $0.69 \pm 0.01$\\
\hline
\end{tabular}
 }
\label{tab:citeseer-dp-ind}
\end{table}

==> chapters/appendices/Nl_1-2_TwitchDE.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the inductive setting using the rare F1 score on Twitch-DE Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $ - $ & $0.55 \pm 0.0$ & $0.43 \pm 0.04$\\
2.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $0.56 \pm 0.0$ & $0.55 \pm 0.0$ & $0.43 \pm 0.04$\\
3.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $ - $ & $0.55 \pm 0.0$ & $0.44 \pm 0.04$\\
4.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $0.56 \pm 0.0$ & $0.55 \pm 0.0$ & $0.46 \pm 0.03$\\
5.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $ - $ & $0.55 \pm 0.0$ & $0.49 \pm 0.03$\\
6.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $0.56 \pm 0.0$ & $0.55 \pm 0.0$ & $0.51 \pm 0.02$\\
7.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $ - $ & $0.55 \pm 0.0$ & $0.53 \pm 0.01$\\
8.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $0.56 \pm 0.0$ & $0.55 \pm 0.0$ & $0.54 \pm 0.01$\\
9.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $ - $ & $0.55 \pm 0.0$ & $0.54 \pm 0.01$\\
10.0 & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $0.56 \pm 0.0$ & $0.55 \pm 0.0$ & $0.55 \pm 0.01$\\
\hline
\end{tabular}
 }
\label{tab:de-dp-ind}
\end{table}


==> chapters/appendices/Nl_1_2_Facebook_page.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the transductive setting using the micro-average F1 score on Facebook Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.74 \pm 0.01$ & $0.78 \pm 0.01$ & $ - $ & $0.93 \pm 0.0$ & $0.3 \pm 0.01$\\
2.0 & $0.74 \pm 0.01$ & $0.8 \pm 0.01$ & $0.8 \pm 0.01$ & $0.93 \pm 0.0$ & $0.3 \pm 0.01$\\
3.0 & $0.74 \pm 0.01$ & $0.81 \pm 0.01$ & $ - $ & $0.93 \pm 0.0$ & $0.3 \pm 0.01$\\
4.0 & $0.74 \pm 0.01$ & $0.82 \pm 0.01$ & $0.83 \pm 0.01$ & $0.93 \pm 0.0$ & $0.3 \pm 0.01$\\
5.0 & $0.74 \pm 0.01$ & $0.82 \pm 0.01$ & $ - $ & $0.93 \pm 0.0$ & $0.35 \pm 0.01$\\
6.0 & $0.74 \pm 0.01$ & $0.82 \pm 0.01$ & $0.85 \pm 0.01$ & $0.93 \pm 0.0$ & $0.47 \pm 0.03$\\
7.0 & $0.74 \pm 0.01$ & $0.82 \pm 0.01$ & $ - $ & $0.93 \pm 0.0$ & $0.63 \pm 0.01$\\
8.0 & $0.74 \pm 0.01$ & $0.83 \pm 0.01$ & $0.85 \pm 0.01$ & $0.93 \pm 0.0$ & $0.74 \pm 0.01$\\
9.0 & $0.74 \pm 0.01$ & $0.83 \pm 0.01$ & $ - $ & $0.93 \pm 0.0$ & $0.81 \pm 0.01$\\
10.0 & $0.74 \pm 0.01$ & $0.83 \pm 0.01$ & $0.86 \pm 0.01$ & $0.93 \pm 0.0$ & $0.85 \pm 0.01$\\
\hline
\end{tabular}
 }
\label{tab:facebook-dp-ind}
\end{table}

==> chapters/appendices/Nl_1_2_Flickr.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the inductive setting using the micro-average F1 score on Flickr Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $ - $ & $0.51 \pm 0.0$ & $0.44 \pm 0.0$\\
2.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $0.48 \pm 0.0$ & $0.51 \pm 0.0$ & $0.44 \pm 0.0$\\
3.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $ - $ & $0.51 \pm 0.0$ & $0.44 \pm 0.0$\\
4.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $0.49 \pm 0.0$ & $0.51 \pm 0.0$ & $0.44 \pm 0.0$\\
5.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $ - $ & $0.51 \pm 0.0$ & $0.44 \pm 0.0$\\
6.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $0.49 \pm 0.0$ & $0.51 \pm 0.0$ & $0.44 \pm 0.0$\\
7.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $ - $ & $0.51 \pm 0.0$ & $0.44 \pm 0.0$\\
8.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $0.49 \pm 0.0$ & $0.51 \pm 0.0$ & $0.45 \pm 0.0$\\
9.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $ - $ & $0.51 \pm 0.0$ & $0.47 \pm 0.0$\\
10.0 & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $0.49 \pm 0.0$ & $0.51 \pm 0.0$ & $0.49 \pm 0.0$\\
\hline
\end{tabular}
 }
\label{tab:flickr-dp-ind}
\end{table}

==> chapters/appendices/Nl_1_2_TwitchENGB.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the inductive setting using the rare F1 score on Twitch-ENGB Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $ - $ & $0.6 \pm 0.0$ & $0.6 \pm 0.01$\\
2.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.01$\\
3.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $ - $ & $0.6 \pm 0.0$ & $0.6 \pm 0.01$\\
4.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.01$\\
5.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $ - $ & $0.6 \pm 0.0$ & $0.6 \pm 0.01$\\
6.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.01$\\
7.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $ - $ & $0.6 \pm 0.0$ & $0.6 \pm 0.01$\\
8.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.01$\\
9.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.01$ & $ - $ & $0.6 \pm 0.0$ & $0.6 \pm 0.01$\\
10.0 & $0.6 \pm 0.0$ & $0.6 \pm 0.01$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$\\
\hline
\end{tabular}
 }
\label{tab:engb-dp-ind}
\end{table}


==> chapters/appendices/Nl_1_2_TwitchFR.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the inductive setting using the rare F1 score on Twitch-FR Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.37 \pm 0.01$ & $0.37 \pm 0.01$ & $ - $ & $0.43 \pm 0.02$ & $0.39 \pm 0.07$\\
2.0 & $0.37 \pm 0.01$ & $0.37 \pm 0.01$ & $0.37 \pm 0.01$ & $0.43 \pm 0.02$ & $0.39 \pm 0.07$\\
3.0 & $0.37 \pm 0.01$ & $0.37 \pm 0.02$ & $ - $ & $0.43 \pm 0.02$ & $0.37 \pm 0.07$\\
4.0 & $0.37 \pm 0.01$ & $0.37 \pm 0.02$ & $0.36 \pm 0.01$ & $0.43 \pm 0.02$ & $0.34 \pm 0.09$\\
5.0 & $0.37 \pm 0.01$ & $0.36 \pm 0.02$ & $ - $ & $0.43 \pm 0.02$ & $0.32 \pm 0.1$\\
6.0 & $0.37 \pm 0.01$ & $0.37 \pm 0.02$ & $0.37 \pm 0.01$ & $0.43 \pm 0.02$ & $0.32 \pm 0.08$\\
7.0 & $0.37 \pm 0.01$ & $0.37 \pm 0.01$ & $ - $ & $0.43 \pm 0.02$ & $0.33 \pm 0.08$\\
8.0 & $0.37 \pm 0.01$ & $0.36 \pm 0.02$ & $0.36 \pm 0.01$ & $0.43 \pm 0.02$ & $0.37 \pm 0.06$\\
9.0 & $0.37 \pm 0.01$ & $0.36 \pm 0.02$ & $ - $ & $0.43 \pm 0.02$ & $0.37 \pm 0.06$\\
10.0 & $0.37 \pm 0.01$ & $0.37 \pm 0.01$ & $0.37 \pm 0.02$ & $0.43 \pm 0.02$ & $0.4 \pm 0.04$\\
\hline
\end{tabular}
 }
\label{tab:fr-dp-ind}
\end{table}


==> chapters/appendices/Nl_1_2_TwitchPTBR.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the inductive setting using the rare F1 score on Twitch-PTBR Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $ - $ & $0.45 \pm 0.01$ & $0.43 \pm 0.03$\\
2.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $0.45 \pm 0.01$ & $0.44 \pm 0.03$\\
3.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.01$ & $ - $ & $0.45 \pm 0.01$ & $0.44 \pm 0.03$\\
4.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $0.45 \pm 0.01$ & $0.45 \pm 0.04$\\
5.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.01$ & $ - $ & $0.45 \pm 0.01$ & $0.45 \pm 0.04$\\
6.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $0.34 \pm 0.01$ & $0.45 \pm 0.01$ & $0.46 \pm 0.03$\\
7.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $ - $ & $0.45 \pm 0.01$ & $0.46 \pm 0.03$\\
8.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $0.34 \pm 0.02$ & $0.45 \pm 0.01$ & $0.46 \pm 0.03$\\
9.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $ - $ & $0.45 \pm 0.01$ & $0.45 \pm 0.02$\\
10.0 & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $0.34 \pm 0.02$ & $0.45 \pm 0.01$ & $0.45 \pm 0.02$\\
\hline
\end{tabular}
 }
\label{tab:ptbr-dp-ind}
\end{table}


==> chapters/appendices/Nl_1_2_TwitchRU.tex <==
\begin{table}[t]
\centering
\caption{Node classification results for the inductive setting using the rare F1 score on Twitch-RU Dataset.}

 \resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
\toprule
Epsilon &  \mlp  & \toola & \toolb  & \gcn  &  \dpgcn \\\hline

1.0 & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $ - $ & $0.31 \pm 0.01$ & $0.28 \pm 0.02$\\
2.0 & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.31 \pm 0.01$ & $0.29 \pm 0.02$\\
3.0 & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $ - $ & $0.31 \pm 0.01$ & $0.28 \pm 0.02$\\
4.0 & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.31 \pm 0.01$ & $0.29 \pm 0.02$\\
5.0 & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $ - $ & $0.31 \pm 0.01$ & $0.29 \pm 0.02$\\
6.0 & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.31 \pm 0.01$ & $0.29 \pm 0.02$\\
7.0 & $0.27 \pm 0.01$ & $0.28 \pm 0.01$ & $ - $ & $0.31 \pm 0.01$ & $0.3 \pm 0.02$\\
8.0 & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.31 \pm 0.01$ & $0.3 \pm 0.02$\\
9.0 & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $ - $ & $0.31 \pm 0.01$ & $0.3 \pm 0.02$\\
10.0 & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.27 \pm 0.01$ & $0.31 \pm 0.01$ & $0.31 \pm 0.01$\\
\hline
\end{tabular}
 }
\label{tab:ru-dp-ind}
\end{table}


==> chapters/appendices/attack.tex <==
\begin{table*}[th!]
   \centering
\caption{Attack in Transductive Setting}

   \resizebox{\textwidth}{!}{
%\toprule
\begin{tabular}{c c c c c c c c c c } 
     \toprule       Model & Epsilon   & \multicolumn{2}{c}{Citeseer}  & \multicolumn{2}{c}{Cora}  & \multicolumn{2}{c}{Facebook}  & \multicolumn{2}{c}{Pubmed}               \\
     \hline 
                  &           &   \baselineAttack & \sotaAttack                 &   \baselineAttack & \sotaAttack              &   \baselineAttack & \sotaAttack                &   \baselineAttack & \sotaAttack                             \\
    \hline
\mlp
& $0.0$& $0.78 \pm 0.02$& $0.50 \pm 0.00$& $0.74 \pm 0.02$& $0.50 \pm 0.00$& $0.81 \pm 0.02$& $0.50 \pm 0.00$& $0.75 \pm 0.02$& $0.50 \pm 0.00$\\

\hline
\gcn
& $0.0$& $0.96 \pm 0.00$& $1.00 \pm 0.00$& $0.94 \pm 0.01$& $1.00 \pm 0.00$& $0.88 \pm 0.01$& $1.00 \pm 0.00$& $0.87 \pm 0.01$& $1.00 \pm 0.00$\\

\hline
\multirow{11}{*}{\dpgcn}
& $1.0$& $0.61 \pm 0.03$& $0.50 \pm 0.00$& $0.58 \pm 0.02$& $0.50 \pm 0.00$& $0.50 \pm 0.01$& $0.50 \pm 0.00$& $0.58 \pm 0.02$& $0.50 \pm 0.00$\\

& $2.0$& $0.62 \pm 0.03$& $0.50 \pm 0.00$& $0.60 \pm 0.01$& $0.50 \pm 0.00$& $0.50 \pm 0.02$& $0.50 \pm 0.00$& $0.60 \pm 0.01$& $0.50 \pm 0.00$\\

& $3.0$& $0.62 \pm 0.03$& $0.51 \pm 0.00$& $0.59 \pm 0.01$& $0.51 \pm 0.00$& $0.51 \pm 0.02$& $0.50 \pm 0.00$& $0.58 \pm 0.02$& $0.50 \pm 0.00$\\

& $4.0$& $0.64 \pm 0.02$& $0.52 \pm 0.00$& $0.62 \pm 0.02$& $0.53 \pm 0.00$& $0.50 \pm 0.02$& $0.51 \pm 0.00$& $0.60 \pm 0.03$& $0.50 \pm 0.00$\\

& $5.0$& $0.67 \pm 0.02$& $0.55 \pm 0.01$& $0.67 \pm 0.02$& $0.59 \pm 0.01$& $0.54 \pm 0.01$& $0.54 \pm 0.01$& $0.61 \pm 0.02$& $0.51 \pm 0.00$\\

& $6.0$& $0.73 \pm 0.02$& $0.63 \pm 0.01$& $0.76 \pm 0.01$& $0.69 \pm 0.01$& $0.63 \pm 0.02$& $0.66 \pm 0.02$& $0.62 \pm 0.02$& $0.54 \pm 0.00$\\

& $7.0$& $0.81 \pm 0.02$& $0.75 \pm 0.01$& $0.84 \pm 0.01$& $0.82 \pm 0.00$& $0.72 \pm 0.01$& $0.82 \pm 0.01$& $0.66 \pm 0.02$& $0.59 \pm 0.01$\\

& $8.0$& $0.88 \pm 0.01$& $0.85 \pm 0.01$& $0.88 \pm 0.01$& $0.90 \pm 0.00$& $0.79 \pm 0.02$& $0.92 \pm 0.01$& $0.73 \pm 0.01$& $0.70 \pm 0.01$\\

& $9.0$& $0.92 \pm 0.01$& $0.91 \pm 0.01$& $0.9 \pm 0.01$& $0.95 \pm 0.00$& $0.83 \pm 0.01$& $0.96 \pm 0.01$& $0.78 \pm 0.03$& $0.82 \pm 0.01$\\

& $10.0$& $0.93 \pm 0.01$& $0.95 \pm 0.01$& $0.92 \pm 0.01$& $0.97 \pm 0.00$& $0.85 \pm 0.01$& $0.98 \pm 0.00$& $0.81 \pm 0.01$& $0.89 \pm 0.01$\\

\hline
\multirow{11}{*}{\toola}
& $0.0$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.80 \pm 0.01$& $0.50 \pm 0.00$\\

& $1.0$& $0.77 \pm 0.03$& $0.50 \pm 0.00$& $0.72 \pm 0.02$& $0.50 \pm 0.00$& $0.82 \pm 0.01$& $0.50 \pm 0.00$& $0.76 \pm 0.01$& $0.50 \pm 0.00$\\

& $2.0$& $0.81 \pm 0.01$& $0.50 \pm 0.00$& $0.78 \pm 0.02$& $0.50 \pm 0.00$& $0.83 \pm 0.01$& $0.50 \pm 0.00$& $0.77 \pm 0.00$& $0.50 \pm 0.00$\\

& $3.0$& $0.83 \pm 0.02$& $0.50 \pm 0.00$& $0.82 \pm 0.01$& $0.50 \pm 0.00$& $0.84 \pm 0.01$& $0.50 \pm 0.00$& $0.79 \pm 0.00$& $0.50 \pm 0.00$\\

& $4.0$& $0.84 \pm 0.02$& $0.50 \pm 0.00$& $0.83 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.78 \pm 0.02$& $0.50 \pm 0.00$\\

& $5.0$& $0.84 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.02$& $0.50 \pm 0.00$& $0.84 \pm 0.01$& $0.50 \pm 0.00$& $0.78 \pm 0.01$& $0.50 \pm 0.00$\\

& $6.0$& $0.84 \pm 0.02$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.79 \pm 0.01$& $0.43 \pm 0.01$\\

& $7.0$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.02$& $0.50 \pm 0.00$& $0.79 \pm 0.01$& $0.50 \pm 0.00$\\

& $8.0$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.78 \pm 0.02$& $0.50 \pm 0.00$\\

& $9.0$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.80 \pm 0.01$& $0.50 \pm 0.00$\\

& $10.0$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.79 \pm 0.02$& $0.50 \pm 0.00$\\

\hline
\multirow{10}{*}{\toolb}
& $0.0$& $0.89 \pm 0.01$& $0.50 \pm 0.00$& $0.88 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.82 \pm 0.01$& $0.50 \pm 0.00$\\

& $1.0$& $0.75 \pm 0.02$& $0.50 \pm 0.00$& $0.74 \pm 0.01$& $0.50 \pm 0.00$& $0.83 \pm 0.01$& $0.50 \pm 0.00$& $0.75 \pm 0.01$& $0.50 \pm 0.00$\\

& $2.0$& $0.81 \pm 0.02$& $0.50 \pm 0.00$& $0.81 \pm 0.01$& $0.50 \pm 0.00$& $0.84 \pm 0.02$& $0.50 \pm 0.00$& $0.78 \pm 0.01$& $0.50 \pm 0.00$\\

& $3.0$& $0.83 \pm 0.02$& $0.50 \pm 0.00$& $0.84 \pm 0.01$& $0.50 \pm 0.00$& $0.84 \pm 0.01$& $0.50 \pm 0.00$& $0.79 \pm 0.01$& $0.50 \pm 0.00$\\

& $4.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.80 \pm 0.00$& $0.50 \pm 0.00$\\

& $5.0$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.80 \pm 0.01$& $0.50 \pm 0.00$\\

& $6.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.79 \pm 0.02$& $0.50 \pm 0.00$\\

& $7.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.84 \pm 0.01$& $0.50 \pm 0.00$& $0.80 \pm 0.01$& $0.50 \pm 0.00$\\

& $8.0$& $0.88 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.02$& $0.50 \pm 0.00$& $0.81 \pm 0.01$& $0.50 \pm 0.00$\\

& $9.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.80 \pm 0.01$& $0.50 \pm 0.00$\\

& $10.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.80 \pm 0.01$& $0.50 \pm 0.00$\\

\hline
% \multirow{11}{*}{\toolc}
% & $0.0$& $0.90 \pm 0.01$& $0.50 \pm 0.00$& $0.89 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.82 \pm 0.01$& $0.50 \pm 0.00$\\

% & $1.0$& $0.73 \pm 0.02$& $0.50 \pm 0.00$& $0.75 \pm 0.03$& $0.50 \pm 0.00$& $0.83 \pm 0.01$& $0.50 \pm 0.00$& $0.76 \pm 0.02$& $0.50 \pm 0.00$\\

% & $2.0$& $0.81 \pm 0.02$& $0.50 \pm 0.00$& $0.81 \pm 0.01$& $0.50 \pm 0.00$& $0.84 \pm 0.01$& $0.50 \pm 0.00$& $0.78 \pm 0.01$& $0.50 \pm 0.00$\\

% & $3.0$& $0.84 \pm 0.02$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.79 \pm 0.01$& $0.50 \pm 0.00$\\

% & $4.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.02$& $0.50 \pm 0.00$& $0.80 \pm 0.02$& $0.50 \pm 0.00$\\

% & $5.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.00$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.80 \pm 0.01$& $0.50 \pm 0.00$\\

% & $6.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.81 \pm 0.01$& $0.50 \pm 0.00$\\

% & $7.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.87 \pm 0.00$& $0.50 \pm 0.00$& $0.85 \pm 0.01$& $0.50 \pm 0.00$& $0.81 \pm 0.01$& $0.50 \pm 0.00$\\

% & $8.0$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.81 \pm 0.01$& $0.50 \pm 0.00$\\

% & $9.0$& $0.9 \pm 0.01$& $0.50 \pm 0.00$& $0.87 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.82 \pm 0.01$& $0.50 \pm 0.00$\\

% & $10.0$& $0.88 \pm 0.01$& $0.50 \pm 0.00$& $0.88 \pm 0.01$& $0.50 \pm 0.00$& $0.86 \pm 0.01$& $0.50 \pm 0.00$& $0.81 \pm 0.02$& $0.50 \pm 0.00$\\

% \hline
\end{tabular}
       }
\label{tab:hyperparameters}
       \end{table*}


==> chapters/appendices/attack_engb.tex <==
\begin{table*}[t]
   \centering
\caption{Attack Table in Inductive Setting in Twitch-ENGB Dataset.}

   \resizebox{\textwidth}{!}{

\begin{tabular}{c c c c c c c c c c c c c} 
            Model & Epsilon   & \multicolumn{2}{c}{\baselineAttack}  & \multicolumn{2}{c}{\sotaAttack} \\
    \hline 
                  &           &  lo   & hi & baseline                 &   lo & hi & baseline    \\
    \hline
GCN
& $0$& $0.65\pm0.08$& $0.55\pm0.02$&$0.56\pm0.01$&$1.0\pm0.0$&$0.99\pm0.0$&$1.0\pm0.0$\\

\hline
\multirow{10}{*}{DPGCN}
& $1$& $0.57\pm0.09$& $0.51\pm0.01$&$0.49\pm0.02$&$0.51\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $2$& $0.56\pm0.08$& $0.51\pm0.01$&$0.47\pm0.03$&$0.48\pm0.02$&$0.51\pm0.01$&$0.5\pm0.0$\\

& $3$& $0.55\pm0.08$& $0.5\pm0.01$&$0.47\pm0.01$&$0.47\pm0.01$&$0.52\pm0.0$&$0.51\pm0.01$\\

& $4$& $0.53\pm0.1$& $0.51\pm0.02$&$0.48\pm0.05$&$0.53\pm0.05$&$0.55\pm0.01$&$0.55\pm0.02$\\

& $5$& $0.49\pm0.07$& $0.52\pm0.01$&$0.49\pm0.01$&$0.56\pm0.06$&$0.64\pm0.01$&$0.64\pm0.03$\\

& $6$& $0.47\pm0.08$& $0.52\pm0.02$&$0.5\pm0.03$&$0.63\pm0.09$&$0.78\pm0.01$&$0.77\pm0.02$\\

& $7$& $0.57\pm0.05$& $0.54\pm0.01$&$0.52\pm0.03$&$0.79\pm0.07$&$0.9\pm0.01$&$0.89\pm0.01$\\

& $8$& $0.49\pm0.07$& $0.54\pm0.01$&$0.51\pm0.04$&$0.87\pm0.07$&$0.95\pm0.0$&$0.95\pm0.01$\\

& $9$& $0.56\pm0.03$& $0.54\pm0.01$&$0.52\pm0.02$&$0.92\pm0.05$&$0.96\pm0.0$&$0.97\pm0.0$\\

& $10$& $0.58\pm0.03$& $0.54\pm0.02$&$0.53\pm0.01$&$0.94\pm0.05$&$0.98\pm0.0$&$0.98\pm0.01$\\

\hline
\multirow{11}{*}{\toola}
& $0$& $0.49\pm0.03$& $0.52\pm0.01$&$0.49\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $1$& $0.49\pm0.1$& $0.51\pm0.0$&$0.48\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $2$& $0.52\pm0.09$& $0.51\pm0.01$&$0.47\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $3$& $0.51\pm0.09$& $0.52\pm0.01$&$0.49\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $4$& $0.46\pm0.08$& $0.51\pm0.01$&$0.46\pm0.04$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $5$& $0.51\pm0.08$& $0.51\pm0.01$&$0.49\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $6$& $0.52\pm0.12$& $0.51\pm0.01$&$0.49\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $7$& $0.49\pm0.07$& $0.52\pm0.0$&$0.5\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $8$& $0.49\pm0.12$& $0.51\pm0.0$&$0.49\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $9$& $0.5\pm0.08$& $0.51\pm0.0$&$0.5\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $10$& $0.47\pm0.06$& $0.52\pm0.01$&$0.49\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

\hline
\multirow{11}{*}{\toolb}
& $0$& $0.5\pm0.03$& $0.5\pm0.01$&$0.48\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $1$& $0.48\pm0.09$& $0.51\pm0.01$&$0.48\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $2$& $0.51\pm0.05$& $0.51\pm0.01$&$0.47\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $3$& $0.47\pm0.06$& $0.51\pm0.0$&$0.48\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $4$& $0.53\pm0.06$& $0.52\pm0.01$&$0.48\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $5$& $0.51\pm0.05$& $0.51\pm0.0$&$0.49\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $6$& $0.48\pm0.08$& $0.51\pm0.0$&$0.47\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $7$& $0.52\pm0.03$& $0.51\pm0.01$&$0.49\pm0.04$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $8$& $0.47\pm0.05$& $0.52\pm0.01$&$0.48\pm0.01$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $9$& $0.47\pm0.09$& $0.51\pm0.0$&$0.48\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $10$& $0.47\pm0.07$& $0.52\pm0.01$&$0.48\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

\hline
\multirow{11}{*}{\toolc}
& $0$& $0.52\pm0.04$& $0.52\pm0.01$&$0.48\pm0.04$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $1$& $0.49\pm0.07$& $0.51\pm0.01$&$0.47\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $2$& $0.48\pm0.1$& $0.52\pm0.01$&$0.49\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $3$& $0.47\pm0.08$& $0.51\pm0.01$&$0.47\pm0.04$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $4$& $0.48\pm0.1$& $0.51\pm0.01$&$0.47\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $5$& $0.51\pm0.11$& $0.52\pm0.01$&$0.5\pm0.01$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $6$& $0.44\pm0.09$& $0.52\pm0.01$&$0.48\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $7$& $0.49\pm0.1$& $0.52\pm0.01$&$0.48\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $8$& $0.5\pm0.09$& $0.52\pm0.0$&$0.48\pm0.02$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $9$& $0.46\pm0.1$& $0.52\pm0.01$&$0.47\pm0.04$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

& $10$& $0.46\pm0.09$& $0.52\pm0.01$&$0.47\pm0.03$&$0.5\pm0.0$&$0.5\pm0.0$&$0.5\pm0.0$\\

\hline
\end{tabular}
       }
\label{tab:hyperparameters}
       \end{table*}


==> chapters/appendices/ind_attack_1.tex <==
\begin{table*}[th!]
\centering
\caption{Attack in Transductive Setting}
\resizebox{\textwidth}{!}{
\begin{tabular}{c c c c c c c c }
\toprule
Model & Epsilon & \multicolumn{2}{c}{TwitchDE} & \multicolumn{2}{c}{TwitchPTBR} & \multicolumn{2}{c}{TwitchRU}\\\hline
 & & \baselineAttack & \sotaAttack & \baselineAttack & \sotaAttack & \baselineAttack & \sotaAttack\\\hline

\mlp
& $\infty$ & $0.5 \pm 0.01$ & $0.5 \pm 0.0$ & $0.45 \pm 0.01$ & $0.5 \pm 0.0$ & $0.49 \pm 0.03$ & $0.5 \pm 0.0$\\\hline
\gcn
& $\infty$ & $0.54 \pm 0.02$ & $1.0 \pm 0.0$ & $0.57 \pm 0.05$ & $0.99 \pm 0.0$ & $0.52 \pm 0.01$ & $0.99 \pm 0.0$\\\hline
\toola
& $\infty$ & $0.5 \pm 0.02$ & $0.5 \pm 0.0$ & $0.46 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.01$ & $0.5 \pm 0.0$\\\hline
\toolb
& $\infty$ & $0.5 \pm 0.01$ & $0.5 \pm 0.0$ & $0.45 \pm 0.03$ & $0.5 \pm 0.0$ & $0.48 \pm 0.01$ & $0.5 \pm 0.0$\\\hline

\multirow{10}{*}{\dpgcn}
& $1.0$ & $0.48 \pm 0.02$ & $0.54 \pm 0.02$ & $0.52 \pm 0.02$ & $0.56 \pm 0.01$ & $0.49 \pm 0.02$ & $0.51 \pm 0.03$\\

& $2.0$ & $0.5 \pm 0.03$ & $0.57 \pm 0.01$ & $0.52 \pm 0.02$ & $0.62 \pm 0.0$ & $0.49 \pm 0.02$ & $0.53 \pm 0.04$\\

& $3.0$ & $0.5 \pm 0.02$ & $0.6 \pm 0.03$ & $0.53 \pm 0.02$ & $0.74 \pm 0.02$ & $0.5 \pm 0.02$ & $0.6 \pm 0.04$\\

& $4.0$ & $0.52 \pm 0.01$ & $0.71 \pm 0.01$ & $0.54 \pm 0.03$ & $0.85 \pm 0.01$ & $0.52 \pm 0.02$ & $0.7 \pm 0.03$\\

& $5.0$ & $0.51 \pm 0.02$ & $0.8 \pm 0.01$ & $0.55 \pm 0.04$ & $0.93 \pm 0.01$ & $0.49 \pm 0.02$ & $0.82 \pm 0.02$\\

& $6.0$ & $0.52 \pm 0.02$ & $0.91 \pm 0.01$ & $0.54 \pm 0.03$ & $0.96 \pm 0.01$ & $0.52 \pm 0.02$ & $0.91 \pm 0.01$\\

& $7.0$ & $0.53 \pm 0.02$ & $0.96 \pm 0.01$ & $0.55 \pm 0.01$ & $0.95 \pm 0.0$ & $-1.0 \pm -1.0$ & $-1.0 \pm -1.0$\\

& $8.0$ & $0.52 \pm 0.02$ & $0.97 \pm 0.0$ & $0.57 \pm 0.02$ & $0.98 \pm 0.0$ & $0.54 \pm 0.01$ & $0.97 \pm 0.01$\\

& $9.0$ & $0.55 \pm 0.02$ & $0.98 \pm 0.0$ & $0.55 \pm 0.03$ & $0.98 \pm 0.0$ & $0.52 \pm 0.02$ & $0.98 \pm 0.01$\\

& $10.0$ & $0.54 \pm 0.01$ & $0.99 \pm 0.0$ & $0.57 \pm 0.03$ & $0.98 \pm 0.0$ & $0.52 \pm 0.01$ & $0.99 \pm 0.0$\\
\hline

\multirow{10}{*}{\toola}
& $1.0$ & $0.49 \pm 0.01$ & $0.5 \pm 0.0$ & $0.47 \pm 0.04$ & $0.5 \pm 0.0$ & $0.51 \pm 0.02$ & $0.5 \pm 0.0$\\

& $2.0$ & $0.5 \pm 0.01$ & $0.5 \pm 0.0$ & $0.47 \pm 0.04$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $3.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.46 \pm 0.02$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $4.0$ & $0.5 \pm 0.01$ & $0.5 \pm 0.0$ & $0.46 \pm 0.02$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $5.0$ & $0.49 \pm 0.01$ & $0.5 \pm 0.0$ & $0.47 \pm 0.01$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $6.0$ & $0.5 \pm 0.01$ & $0.5 \pm 0.0$ & $0.47 \pm 0.03$ & $0.5 \pm 0.0$ & $0.51 \pm 0.02$ & $0.5 \pm 0.0$\\

& $7.0$ & $0.49 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $8.0$ & $0.49 \pm 0.03$ & $0.5 \pm 0.0$ & $0.46 \pm 0.03$ & $0.5 \pm 0.0$ & $0.5 \pm 0.02$ & $0.5 \pm 0.0$\\

& $9.0$ & $0.49 \pm 0.01$ & $0.5 \pm 0.0$ & $0.47 \pm 0.04$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $10.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.45 \pm 0.02$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\
\hline

\multirow{10}{*}{\toolb}
& $1.0$ & $0.49 \pm 0.02$ & $0.5 \pm 0.0$ & $0.46 \pm 0.02$ & $0.5 \pm 0.0$ & $0.5 \pm 0.01$ & $0.5 \pm 0.0$\\

& $2.0$ & $-1.0 \pm -1.0$ & $-1.0 \pm -1.0$ & $0.46 \pm 0.03$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $3.0$ & $0.5 \pm 0.02$ & $0.5 \pm 0.0$ & $0.46 \pm 0.03$ & $0.5 \pm 0.0$ & $0.51 \pm 0.02$ & $0.5 \pm 0.0$\\

& $4.0$ & $0.5 \pm 0.01$ & $0.5 \pm 0.0$ & $0.47 \pm 0.02$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $5.0$ & $0.5 \pm 0.01$ & $0.5 \pm 0.0$ & $0.46 \pm 0.02$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $6.0$ & $0.5 \pm 0.02$ & $0.5 \pm 0.0$ & $0.45 \pm 0.03$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $7.0$ & $0.49 \pm 0.02$ & $0.5 \pm 0.0$ & $0.45 \pm 0.03$ & $0.5 \pm 0.0$ & $0.51 \pm 0.01$ & $0.5 \pm 0.0$\\

& $8.0$ & $0.5 \pm 0.02$ & $0.5 \pm 0.0$ & $0.46 \pm 0.03$ & $0.5 \pm 0.0$ & $0.51 \pm 0.02$ & $0.5 \pm 0.0$\\

& $9.0$ & $0.5 \pm 0.02$ & $0.5 \pm 0.0$ & $0.45 \pm 0.04$ & $0.5 \pm 0.0$ & $0.51 \pm 0.02$ & $0.5 \pm 0.0$\\

& $10.0$ & $0.5 \pm 0.02$ & $0.5 \pm 0.0$ & $0.47 \pm 0.02$ & $0.5 \pm 0.0$ & $0.51 \pm 0.02$ & $0.5 \pm 0.0$\\
\hline

\end{tabular}
}
\label{tab:ind_1_attack}
\end{table*}


==> chapters/appendices/ind_attack_2.tex <==
\begin{table*}[th!]
\centering
\caption{Attack in Transductive Setting}
\resizebox{\textwidth}{!}{
\begin{tabular}{c c c c c c c c }
\toprule
Model & Epsilon & \multicolumn{2}{c}{TwitchENGB} & \multicolumn{2}{c}{TwitchFR} & \multicolumn{2}{c}{Flickr}\\\hline
 & & \baselineAttack & \sotaAttack & \baselineAttack & \sotaAttack & \baselineAttack & \sotaAttack\\\hline

\mlp
& $\infty$ & $0.47 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.5 \pm 0.05$ & $0.5 \pm 0.0$\\\hline
\gcn
& $\infty$ & $0.54 \pm 0.02$ & $1.0 \pm 0.0$ & $0.52 \pm 0.02$ & $0.99 \pm 0.0$ & $0.61 \pm 0.07$ & $1.0 \pm 0.0$\\\hline
\toola
& $\infty$ & $0.47 \pm 0.03$ & $0.5 \pm 0.0$ & $0.49 \pm 0.04$ & $0.5 \pm 0.0$ & $0.54 \pm 0.08$ & $0.5 \pm 0.0$\\\hline
\toolb
& $\infty$ & $0.49 \pm 0.03$ & $0.5 \pm 0.0$ & $0.49 \pm 0.02$ & $0.5 \pm 0.0$ & $0.57 \pm 0.08$ & $0.5 \pm 0.0$\\\hline

\multirow{10}{*}{\dpgcn}
& $1.0$ & $0.5 \pm 0.02$ & $0.5 \pm 0.01$ & $0.51 \pm 0.01$ & $0.53 \pm 0.03$ & $0.49 \pm 0.06$ & $0.5 \pm 0.0$\\

& $2.0$ & $0.48 \pm 0.01$ & $0.5 \pm 0.01$ & $0.53 \pm 0.02$ & $0.57 \pm 0.03$ & $0.49 \pm 0.06$ & $0.5 \pm 0.0$\\

& $3.0$ & $0.47 \pm 0.02$ & $0.51 \pm 0.02$ & $0.51 \pm 0.03$ & $0.64 \pm 0.03$ & $0.49 \pm 0.06$ & $0.5 \pm 0.0$\\

& $4.0$ & $0.48 \pm 0.05$ & $0.55 \pm 0.03$ & $0.51 \pm 0.01$ & $0.74 \pm 0.03$ & $0.53 \pm 0.08$ & $0.5 \pm 0.0$\\

& $5.0$ & $0.48 \pm 0.01$ & $0.66 \pm 0.02$ & $0.52 \pm 0.02$ & $0.86 \pm 0.02$ & $0.54 \pm 0.07$ & $0.5 \pm 0.0$\\

& $6.0$ & $0.5 \pm 0.03$ & $0.79 \pm 0.02$ & $0.52 \pm 0.04$ & $0.92 \pm 0.01$ & $0.57 \pm 0.1$ & $0.52 \pm 0.02$\\

& $7.0$ & $0.5 \pm 0.04$ & $0.91 \pm 0.01$ & $0.52 \pm 0.02$ & $0.96 \pm 0.01$ & $0.56 \pm 0.09$ & $0.56 \pm 0.04$\\

& $8.0$ & $0.49 \pm 0.03$ & $0.95 \pm 0.0$ & $0.51 \pm 0.02$ & $0.97 \pm 0.0$ & $0.61 \pm 0.09$ & $0.62 \pm 0.08$\\

& $9.0$ & $0.52 \pm 0.02$ & $0.97 \pm 0.01$ & $0.52 \pm 0.02$ & $0.98 \pm 0.0$ & $0.62 \pm 0.09$ & $0.74 \pm 0.03$\\

& $10.0$ & $0.53 \pm 0.04$ & $0.98 \pm 0.01$ & $0.53 \pm 0.01$ & $0.99 \pm 0.0$ & $0.61 \pm 0.08$ & $0.87 \pm 0.03$\\
\hline

\multirow{10}{*}{\toola}
& $1.0$ & $0.47 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.6 \pm 0.07$ & $0.5 \pm 0.0$\\

& $2.0$ & $0.47 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.01$ & $0.5 \pm 0.0$ & $0.61 \pm 0.05$ & $0.5 \pm 0.0$\\

& $3.0$ & $0.49 \pm 0.02$ & $0.5 \pm 0.0$ & $0.46 \pm 0.03$ & $0.5 \pm 0.0$ & $0.62 \pm 0.05$ & $0.5 \pm 0.0$\\

& $4.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.47 \pm 0.03$ & $0.5 \pm 0.0$ & $0.63 \pm 0.05$ & $0.5 \pm 0.0$\\

& $5.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.47 \pm 0.03$ & $0.5 \pm 0.0$ & $0.63 \pm 0.05$ & $0.5 \pm 0.0$\\

& $6.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.63 \pm 0.05$ & $0.5 \pm 0.0$\\

& $7.0$ & $0.46 \pm 0.03$ & $0.5 \pm 0.0$ & $0.47 \pm 0.03$ & $0.5 \pm 0.0$ & $0.63 \pm 0.05$ & $0.5 \pm 0.0$\\

& $8.0$ & $0.48 \pm 0.03$ & $0.5 \pm 0.0$ & $0.46 \pm 0.03$ & $0.5 \pm 0.0$ & $0.64 \pm 0.05$ & $0.5 \pm 0.0$\\

& $9.0$ & $0.48 \pm 0.03$ & $0.5 \pm 0.0$ & $0.47 \pm 0.01$ & $0.5 \pm 0.0$ & $0.64 \pm 0.05$ & $0.5 \pm 0.0$\\

& $10.0$ & $0.48 \pm 0.03$ & $0.5 \pm 0.0$ & $0.46 \pm 0.03$ & $0.5 \pm 0.0$ & $0.63 \pm 0.05$ & $0.5 \pm 0.0$\\
\hline

\multirow{10}{*}{\toolb}
& $1.0$ & $0.47 \pm 0.03$ & $0.5 \pm 0.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.6 \pm 0.09$ & $0.5 \pm 0.0$\\

& $2.0$ & $0.47 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.6 \pm 0.08$ & $0.5 \pm 0.0$\\

& $3.0$ & $0.49 \pm 0.04$ & $0.5 \pm 0.0$ & $0.47 \pm 0.02$ & $0.5 \pm 0.0$ & $0.64 \pm 0.08$ & $0.5 \pm 0.0$\\

& $4.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.49 \pm 0.02$ & $0.5 \pm 0.0$ & $0.64 \pm 0.09$ & $0.5 \pm 0.0$\\

& $5.0$ & $0.48 \pm 0.03$ & $0.5 \pm 0.0$ & $0.49 \pm 0.0$ & $0.5 \pm 0.0$ & $0.64 \pm 0.1$ & $0.5 \pm 0.0$\\

& $6.0$ & $0.47 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.65 \pm 0.09$ & $0.5 \pm 0.0$\\

& $7.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.49 \pm 0.01$ & $0.5 \pm 0.0$ & $0.64 \pm 0.09$ & $0.5 \pm 0.0$\\

& $8.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.45 \pm 0.03$ & $0.5 \pm 0.0$ & $0.65 \pm 0.09$ & $0.5 \pm 0.0$\\

& $9.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.66 \pm 0.08$ & $0.5 \pm 0.0$\\

& $10.0$ & $0.47 \pm 0.02$ & $0.5 \pm 0.0$ & $0.48 \pm 0.02$ & $0.5 \pm 0.0$ & $0.66 \pm 0.08$ & $0.5 \pm 0.0$\\
\hline

\end{tabular}
}
\label{tab:ind_2_attack}
\end{table*}


==> chapters/appendices/ldp.tex <==
\section{Extending to the LDP setup}
\label{appdx:ldpsetup}

\tool can also be extended for the federated setup where no data provider needs to be trusted with the graph. In this setup, each user (node) in the graph stores their neighbors locally. The data consumer can train \tool on its own servers while the users act as the data providers. Specifically, the data consumer will query every node for their noised degree vectors in each iteration by presenting the clusters from previous iteration. Users can noise their degree vectors locally by adding a noise of $Lap(0, \frac{1}{\epsilon})$ as adding or removing any of their edges may affect only one of their counts by $1$. However the total $\epsilon$ for an edge will still be $2\times\epsilon$ since each edge receives two such queries, one from each affected user.

\paragraph{Privacy risks in LDP setup} The data consumer gets access to all the intermediate logits, gradients, and the degree vectors throughout the training procedure which were not available in the centralized setup. This significantly increases the knowledge that can be used to infer the hidden edge structure. Further, if we do not assume that all users are honest then there is a significant risk for data poisoning attacks by the users~\cite{}. We provide the extension to LDP setup purely from the utility perspective given the recent rising interest in storing data locally. Similar to many existing works~\cite{} if we assume a setup where the users do not want to reveal their exact edges to train a GNN and are honestly following the DP protocol, then \tool may be useful in this setup. We leave studying the repercussions on privacy of the edges if we do not assume honest scenarios to future work.


==> chapters/appendices/utility_attack_efficient_pubmed.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\pubmed, \sotaAttack}
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=triangle,red},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableEfficientPubMed;

\addplot[color = black, dashed, thick] coordinates {(0.5474,0.5) (0.7915,0.5)};
  \addplot[color = black, dashed, thick] coordinates {(0.7292,-1.0) (0.7292, 0.9999)};
  \addplot[color = brown, dashed, thick] coordinates {(0.5474,0.9999) (0.7915,0.9999)};
  \addplot[color = brown, dashed, thick] coordinates {(0.7915,-1.0) (0.7915, 0.9999)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.7292,0.5) rectangle (axis cs:0.7915,0.9999); 


==> data/utils_nondp_ind.tex <==
\begin{table*}[t]
\centering
\caption{Node classification results for the inductive setting using the rare f1 score.}


\begin{tabular}{c c c c c c}
\toprule
Dataset &  \mlp  & \toola & \toolb & \toolc & \gcn\\\hline

\md{Twitch-DE} & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $0.56 \pm 0.0$ & $0.56 \pm 0.0$ & $0.55 \pm 0.0$\\
\md{Twitch-ENGB} & $0.6 \pm 0.0$ & $0.6 \pm 0.01$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$\\
\md{Twitch-FR} & $0.37 \pm 0.01$ & $0.37 \pm 0.02$ & $0.37 \pm 0.01$ & $0.37 \pm 0.02$ & $0.43 \pm 0.02$\\
\md{Twitch-PTBR} & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $0.45 \pm 0.01$\\
\md{Twitch-RU} & $0.27 \pm 0.01$ & $0.27 \pm 0.02$ & $0.28 \pm 0.01$ & $0.27 \pm 0.01$ & $0.31 \pm 0.01$\\
\flickr & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $0.49 \pm 0.0$ & $0.49 \pm 0.0$ & $0.51 \pm 0.0$\\
\hline
\end{tabular}
\label{tab:utlity-nondp-ind}
\end{table*}


==> data/utils_nondp_trans.tex <==
\begin{table*}[t]
\centering
\caption{Node classification results for the transductive setting using the micro-average f1 score.}


\begin{tabular}{c c c c c c}
\toprule
Dataset &  \mlp  & \toola & \toolb & \toolc & \gcn\\\hline

\fbpage & $0.74 \pm 0.01$ & $0.83 \pm 0.01$ & $0.87 \pm 0.01$ & $0.89 \pm 0.01$ & $0.93 \pm 0.01$\\
\seer & $0.6 \pm 0.01$ & $0.65 \pm 0.01$ & $0.67 \pm 0.01$ & $0.68 \pm 0.01$ & $0.72 \pm 0.0$\\
\cora & $0.6 \pm 0.01$ & $0.7 \pm 0.02$ & $0.74 \pm 0.01$ & $0.75 \pm 0.01$ & $0.81 \pm 0.0$\\
\pubmed & $0.72 \pm 0.01$ & $0.75 \pm 0.0$ & $0.75 \pm 0.0$ & $0.76 \pm 0.01$ & $0.79 \pm 0.0$\\
\hline
\end{tabular}
\label{tab:utlity-nondp-trans}
\end{table*}


==> figures/utility_attack_baseline_bipartite.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
legend style={column sep = 1pt, legend columns = 8, legend to name = grouplegend3,},
title={\bipartite, \baselineAttack},
xlabel=Utility F1 score,
ylabel=AUC,
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableBaselineBipartite;
\addlegendentry{\toola}
\addlegendentry{\toolb}
\addlegendentry{\baseline}
\addlegendentry{\mlp}
\addlegendentry{GCN}
\addplot[color = black, dashed, thick] coordinates {(0.5344,0.5056) (1.0,0.5056)};
  \addplot[color = black, dashed, thick] coordinates {(0.5925,0.5003) (0.5925, 0.7608)};
  \addplot[color = brown, dashed, thick] coordinates {(0.5344,0.7608) (1.0,0.7608)};
  \addplot[color = brown, dashed, thick] coordinates {(1.0,0.5003) (1.0, 0.7608)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.5925,0.5056) rectangle (axis cs:1.0,0.7608); 


==> figures/utility_attack_baseline_chameleon.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\chameleon, \baselineAttack}
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableBaselineChameleon;

\addplot[color = black, dashed, thick] coordinates {(0.2243,0.5713) (0.5698,0.5713)};
  \addplot[color = black, dashed, thick] coordinates {(0.4234,0.5003) (0.4234, 0.7722)};
  \addplot[color = brown, dashed, thick] coordinates {(0.2243,0.7722) (0.5698,0.7722)};
  \addplot[color = brown, dashed, thick] coordinates {(0.5698,0.5003) (0.5698, 0.7722)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.4234,0.5713) rectangle (axis cs:0.5698,0.7722); 


==> figures/utility_attack_baseline_citeseer.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\seer, \baselineAttack}
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableBaselineCiteSeer;

\addplot[color = black, dashed, thick] coordinates {(0.3656,0.7788) (0.7153,0.7788)};
  \addplot[color = black, dashed, thick] coordinates {(0.5985,0.6184) (0.5985, 0.9654)};
  \addplot[color = brown, dashed, thick] coordinates {(0.3656,0.9654) (0.7153,0.9654)};
  \addplot[color = brown, dashed, thick] coordinates {(0.7153,0.6184) (0.7153, 0.9654)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.5985,0.7788) rectangle (axis cs:0.7153,0.9654); 


==> figures/utility_attack_baseline_cora.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
legend style={column sep = 1pt, legend columns = 8, legend to name = grouplegend2,},
title={\cora, \baselineAttack},
xlabel=Utility F1 score,
ylabel=AUC,
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableBaselineCora;
\addlegendentry{\toola}
\addlegendentry{\toolb}
\addlegendentry{\baseline}
\addlegendentry{\mlp}
\addlegendentry{GCN}
\addplot[color = black, dashed, thick] coordinates {(0.3357,0.7491) (0.8127,0.7491)};
  \addplot[color = black, dashed, thick] coordinates {(0.5971,0.5866) (0.5971, 0.9387)};
  \addplot[color = brown, dashed, thick] coordinates {(0.3357,0.9387) (0.8127,0.9387)};
  \addplot[color = brown, dashed, thick] coordinates {(0.8127,0.5866) (0.8127, 0.9387)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.5971,0.7491) rectangle (axis cs:0.8127,0.9387); 


==> figures/utility_attack_baseline_facebook_page.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\fbpage, \baselineAttack}
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableBaselineFbpage;

\addplot[color = black, dashed, thick] coordinates {(0.3044,0.8042) (0.928,0.8042)};
  \addplot[color = black, dashed, thick] coordinates {(0.7428,0.4972) (0.7428, 0.8716)};
  \addplot[color = brown, dashed, thick] coordinates {(0.3044,0.8716) (0.928,0.8716)};
  \addplot[color = brown, dashed, thick] coordinates {(0.928,0.4972) (0.928, 0.8716)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.7428,0.8042) rectangle (axis cs:0.928,0.8716); 


==> figures/utility_attack_baseline_pubmed.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\pubmed, \baselineAttack}
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableBaselinePubMed;

\addplot[color = black, dashed, thick] coordinates {(0.5474,0.7504) (0.7915,0.7504)};
  \addplot[color = black, dashed, thick] coordinates {(0.7292,0.5906) (0.7292, 0.8536)};
  \addplot[color = brown, dashed, thick] coordinates {(0.5474,0.8536) (0.7915,0.8536)};
  \addplot[color = brown, dashed, thick] coordinates {(0.7915,0.5906) (0.7915, 0.8536)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.7292,0.7504) rectangle (axis cs:0.7915,0.8536); 


==> figures/utility_attack_efficient_bipartite.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\bipartite, \sotaAttack},
xlabel=Utility F1 score,
ylabel=AUC,
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableEfficientBipartite;

\addplot[color = black, dashed, thick] coordinates {(0.5344,0.4994) (1.0,0.4994)};
  \addplot[color = black, dashed, thick] coordinates {(0.5925,0.4994) (0.5925, 0.9421)};
  \addplot[color = brown, dashed, thick] coordinates {(0.5344,0.9421) (1.0,0.9421)};
  \addplot[color = brown, dashed, thick] coordinates {(1.0,0.4994) (1.0, 0.9421)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.5925,0.4994) rectangle (axis cs:1.0,0.9421); 


==> figures/utility_attack_efficient_chameleon.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\chameleon, \sotaAttack}
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableEfficientChameleon;

\addplot[color = black, dashed, thick] coordinates {(0.2243,0.4998) (0.5698,0.4998)};
  \addplot[color = black, dashed, thick] coordinates {(0.4234,0.4998) (0.4234, 0.9208)};
  \addplot[color = brown, dashed, thick] coordinates {(0.2243,0.9208) (0.5698,0.9208)};
  \addplot[color = brown, dashed, thick] coordinates {(0.5698,0.4998) (0.5698, 0.9208)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.4234,0.4998) rectangle (axis cs:0.5698,0.9208); 


==> figures/utility_attack_efficient_citeseer.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\seer, \sotaAttack}
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableEfficientCiteSeer;

\addplot[color = black, dashed, thick] coordinates {(0.3656,0.5) (0.7153,0.5)};
  \addplot[color = black, dashed, thick] coordinates {(0.5985,0.4998) (0.5985, 0.9988)};
  \addplot[color = brown, dashed, thick] coordinates {(0.3656,0.9988) (0.7153,0.9988)};
  \addplot[color = brown, dashed, thick] coordinates {(0.7153,0.4998) (0.7153, 0.9988)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.5985,0.5) rectangle (axis cs:0.7153,0.9988); 


==> figures/utility_attack_efficient_cora.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\cora, \sotaAttack},
xlabel=Utility F1 score,
ylabel=AUC,
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableEfficientCora;

\addplot[color = black, dashed, thick] coordinates {(0.3357,0.5) (0.8127,0.5)};
  \addplot[color = black, dashed, thick] coordinates {(0.5971,0.5) (0.5971, 0.9992)};
  \addplot[color = brown, dashed, thick] coordinates {(0.3357,0.9992) (0.8127,0.9992)};
  \addplot[color = brown, dashed, thick] coordinates {(0.8127,0.5) (0.8127, 0.9992)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.5971,0.5) rectangle (axis cs:0.8127,0.9992); 


==> figures/utility_attack_efficient_facebook_page.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\fbpage, \sotaAttack}
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableEfficientFbpage;

\addplot[color = black, dashed, thick] coordinates {(0.3044,0.501) (0.928,0.501)};
  \addplot[color = black, dashed, thick] coordinates {(0.7428,0.4986) (0.7428, 0.9987)};
  \addplot[color = brown, dashed, thick] coordinates {(0.3044,0.9987) (0.928,0.9987)};
  \addplot[color = brown, dashed, thick] coordinates {(0.928,0.4986) (0.928, 0.9987)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.7428,0.501) rectangle (axis cs:0.928,0.9987); 


==> figures/utility_attack_efficient_pubmed.tex <==
\nextgroupplot[title style={yshift=-1.2ex},
title={\pubmed, \sotaAttack}
]
\addplot+[scatter,
    only marks,
    scatter/classes={MMLP_nl1={mark=diamond,orange},
                     MMLP_nl2={mark=triangle,red},
                     gcn={mark=o,blue},
                     mlp={mark=+,black},
                     nondp-gcn={mark=+,brown}
                    },
  scatter src=explicit symbolic,
  ] table[x=f1_score_mean, y=auc_score_mean, meta=model]\loadedtableEfficientPubMed;

\addplot[color = black, dashed, thick] coordinates {(0.5474,0.5) (0.7915,0.5)};
  \addplot[color = black, dashed, thick] coordinates {(0.7292,0.5) (0.7292, 0.9999)};
  \addplot[color = brown, dashed, thick] coordinates {(0.5474,0.9999) (0.7915,0.9999)};
  \addplot[color = brown, dashed, thick] coordinates {(0.7915,0.5) (0.7915, 0.9999)};
   \draw [fill=gray,gray,fill opacity=0.4] (axis cs:0.7292,0.5) rectangle (axis cs:0.7915,0.9999); 


==> figures/utility_dp_de_ind.tex <==
% \begin{figure}
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tikzpicture}
\nextgroupplot[title={\md{Twitch-DE}},
        title style={yshift=-1.2ex},
        legend style={nodes={scale=0.8, transform shape}, column sep = 2pt, legend columns = 3, legend to name = grouplegend2,},
        yminorticks=false,
        % adjust the `width' a bit by keeping the default `height'
        ylabel={F1 score},
        % xlabel={$\epsilon$},
        % y label style={font=\Large},
        % x label style={font=\Large},
        % ytick={0.0, 0.2, 0.4, 0.6, 0.8, 1.0},
        % ymin=0.0,
        % ymax=1.2,
        % y tick label style={font=\Large},
        xtick=data,
        xticklabels={1,2,3,4,5,6,7,8,9,10},
        % xticklabels from table={\loadedtableCoraUtilDp}{epsilon_value},
        % x tick label style={font=\Large},
        ymajorgrids,
        log origin=infty,
        % cycle list name = exotic1,
        every axis plot/.append style={thick}
    ]
    % add the data rows
    \foreach \i [evaluate=\i as \j using int(\i+1)] in {1,3,11} {
        \addplot+[sharp plot, very thick, mark=none, error bars/.cd, error bar style={ultra thick}, error mark=none,  y dir=both, y explicit] table [
            x expr=\coordindex,
            y index=\i,
            y error index=\j,
            col sep=comma,
        ] {\loadedtableDEUtilDp};
    }
    \addlegendentry{\mlp}
    \addlegendentry{\gcn}
    \addlegendentry{\toola}
    \foreach \i [evaluate=\i as \j using int(\i+1)] in {13} {
        \addplot+[sharp plot, very thick, mark=none, unbounded coords=discard, error bars/.cd, error bar style={ultra thick}, error mark=none, y dir=both, y explicit] table [
            x expr=\coordindex,
            y index=\i,
            y error index=\j,
            col sep=comma,
        ] {\loadedtableDEUtilDp};
    }
    \addlegendentry{\toolb}
    \foreach \i [evaluate=\i as \j using int(\i+1)] in {9} {
        \addplot+[very thick,dotted, mark=none, color=magenta, error bars/.cd, error bar style={ultra thick}, error mark=none, y dir=both, y explicit] table [
            x expr=\coordindex,
            y index=\i,
            y error index=\j,
            col sep=comma,
        ] {\loadedtableDEUtilDp};
    }
    \addlegendentry{\baseline}

==> tables/parameter_table.tex <==
\begin{table}[t!]
\centering
\caption{Best hyperparameters found via grid search. The column arch represents architecture, lr represents learning rate, hl size is the hidden layer size, \# hls is the number of hidden layers and dr is the dropout rate.}

\resizebox{\columnwidth}{!}{

\begin{tabular}{c c c c c c}
dataset &  arch  & lr & hl size & \# hls & dr \\\hline

\multirow5{*}{\fbpage} & \mlp & 0.05& 64& 3& 0.3\\
 & \gcn & 0.05& 256& 3& 0.1\\
 & \toola & 0.005& 64& 2& 0.1\\
 & \toolb & 0.01& 64& 3& 0.5\\
%  & LPGNET-nl3 & 0.005& 16& 2& 0.5\\
\hline

\multirow5{*}{\pubmed} & \mlp & 0.05& 256& 2& 0.5\\
 & \gcn & 0.05& 64& 2& 0.5\\
 & \toola & 0.001& 256& 2& 0.3\\
 & \toolb & 0.001& 256& 2& 0.1\\
%  & LPGNET-nl3 & 0.001& 256& 2& 0.1\\
\hline

\multirow5{*}{\seer} & \mlp & 0.05& 256& 3& 0.3\\
 & \gcn & 0.05& 256& 2& 0.5\\
 & \toola & 0.01& 256& 2& 0.3\\
 & \toolb & 0.01& 256& 2& 0.5\\
%  & LPGNET-nl3 & 0.01& 256& 2& 0.5\\
\hline

\multirow5{*}{\cora} & \mlp & 0.05& 256& 2& 0.5\\
 & \gcn & 0.05& 256& 2& 0.5\\
 & \toola & 0.001& 64& 2& 0.5\\
 & \toolb & 0.001& 256& 2& 0.5\\
%  & LPGNET-nl3 & 0.001& 256& 2& 0.5\\
\hline

\multirow5{*}{\md{Twitch-[FR,DE,PTBR,ENGB,RU]}}
 & \mlp & 0.01& 256& 3& 0.5\\
 & \gcn & 0.005& 64& 3& 0.1\\
 & \toola & 0.05& 256& 2& 0.1\\
 & \toolb & 0.05& 256& 2& 0.1\\
%  & LPGNET-nl3 & 0.05& 256& 2& 0.1\\
\hline

% \multirow5{*}{\md{Twitch-DE}} & \mlp & 0.005& 256& 3& 0.5\\
%  & \gcn & 0.005& 64& 3& 0.1\\
%  & \toola & 0.05& 256& 2& 0.5\\
%  & \toolb & 0.05& 256& 2& 0.3\\
%  & LPGNET-nl3 & 0.05& 64& 2& 0.5\\
% \hline

% \multirow5{*}{\md{Twitch-PTBR}} & \mlp & 0.01& 256& 3& 0.3\\
%  & \gcn & 0.005& 256& 3& 0.1\\
%  & \toola & 0.05& 256& 2& 0.5\\
%  & \toolb & 0.05& 64& 2& 0.3\\
%  & LPGNET-nl3 & 0.05& 64& 2& 0.1\\
% \hline

% \multirow5{*}{\md{Twitch-ENGB}} & \mlp & 0.01& 256& 3& 0.3\\
%  & \gcn & 0.005& 64& 3& 0.1\\
%  & \toola & 0.05& 256& 2& 0.3\\
%  & \toolb & 0.01& 256& 2& 0.3\\
%  & LPGNET-nl3 & 0.05& 64& 2& 0.5\\
% \hline

% \multirow5{*}{\md{Twitch-RU}} & \mlp & 0.01& 256& 3& 0.5\\
%  & \gcn & 0.005& 64& 3& 0.1\\
%  & \toola & 0.05& 256& 2& 0.1\\
%  & \toolb & 0.05& 256& 2& 0.5\\
%  & LPGNET-nl3 & 0.01& 256& 3& 0.3\\
% \hline

\multirow5{*}{\flickr} & \mlp & 0.0005& 256& 2& 0.2\\
 & \gcn & 0.0005& 256& 2& 0.2\\
 & \toola & 0.0005& 256& 2& 0.2\\
 & \toolb & 0.0005& 256& 2& 0.2\\
%  & LPGNET-nl3 & 0.001& 256& 3& 0.5\\
\hline

\end{tabular}
                }
\label{tab:hyperparameters}
                \end{table}


==> tables/utils_nondp_ind.tex <==
\begin{table*}[t]
\centering
\caption{Node classification results for the inductive setting using the rare f1 score.}


\begin{tabular}{c c c c c c}
\toprule
Dataset &  \mlp  & \toola & \toolb & \toolc & \gcn\\\hline

\md{Twitch-DE} & $0.55 \pm 0.0$ & $0.56 \pm 0.0$ & $0.56 \pm 0.0$ & $0.56 \pm 0.0$ & $0.55 \pm 0.0$\\
\md{Twitch-ENGB} & $0.6 \pm 0.0$ & $0.6 \pm 0.01$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$ & $0.6 \pm 0.0$\\
\md{Twitch-FR} & $0.37 \pm 0.01$ & $0.37 \pm 0.02$ & $0.37 \pm 0.01$ & $0.37 \pm 0.02$ & $0.43 \pm 0.02$\\
\md{Twitch-PTBR} & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $0.34 \pm 0.01$ & $0.34 \pm 0.02$ & $0.45 \pm 0.01$\\
\md{Twitch-RU} & $0.27 \pm 0.01$ & $0.27 \pm 0.02$ & $0.28 \pm 0.01$ & $0.27 \pm 0.01$ & $0.31 \pm 0.01$\\
\flickr & $0.47 \pm 0.0$ & $0.47 \pm 0.0$ & $0.49 \pm 0.0$ & $0.49 \pm 0.0$ & $0.51 \pm 0.0$\\
\hline
\end{tabular}
\label{tab:utlity-nondp-ind}
\end{table*}

